Neuroexplicit Diffusion Models for Inpainting of Optical Flow Fields

Deep learning has revolutionized the field of computer vision by introducing large scale neural networks with millions of parameters. Training these networks requires massive datasets and leads to intransparent models that can fail to generalize. At the other extreme, models designed from partial differential equations (PDEs) embed specialized domain knowledge into mathematical equations and usually rely on few manually chosen hyperparameters. This makes them transparent by construction and if designed and calibrated carefully, they can generalize well to unseen scenarios. In this paper, we show how to bring model- and data-driven approaches together by combining the explicit PDE-based approaches with convolutional neural networks to obtain the best of both worlds. We illustrate a joint architecture for the task of inpainting optical flow fields and show that the combination of model- and data-driven modeling leads to an effective architecture. Our model outperforms both fully explicit and fully data-driven baselines in terms of reconstruction quality, robustness and amount of required training data. Averaging the endpoint error across different mask densities, our method outperforms the explicit baselines by 11-27%, the GAN baseline by 47% and the Probabilisitic Diffusion baseline by 42%. With that, our method sets a new state of the art for inpainting of optical flow fields from random masks.

==> layers/init.tex <==
%\ProvidesPackage{init}
\usetikzlibrary{quotes,arrows.meta}
\usetikzlibrary{positioning}

\def\edgecolorexpl{rgb:blue,4;red,1;green,1;black,3}
\def\edgecolorneur{rgb:blue,4;red,4;green,1;black,3}

\newcommand{\midarrowexpl}{\tikz \draw[-Stealth,line width =1.5mm,draw=\edgecolorexpl] (-0.3,0) -- ++(0.3,0);}

\newcommand{\midarrowneur}{\tikz \draw[-Stealth,line width =0.8mm,draw=\edgecolorneur] (-0.3,0) -- ++(0.3,0);}


\usepackage{Ball}
\usepackage{Box}
\usepackage{RightBandedBox}



==> tmpbib <==
@inproceedings{wasserstein,
  title={Wasserstein generative adversarial networks},
  author={Arjovsky, Martin and Chintala, Soumith and Bottou, L{\'e}on},
  booktitle={International Conference on Machine Learning},
  pages={214--223},
  year={2017},
  organization={PMLR}
},
@article{wganGP,
  title={Improved training of wasserstein gans},
  author={Gulrajani, Ishaan and Ahmed, Faruk and Arjovsky, Martin and Dumoulin, Vincent and Courville, Aaron C},
  journal={Advances in Neural Information Processing Systems},
  volume={30},
  year={2017}
},
@article{layernorm,
  title={Layer normalization},
  author={Ba, Jimmy Lei and Kiros, Jamie Ryan and Hinton, Geoffrey E},
  journal={arXiv preprint arXiv:1607.06450},
  year={2016}
},

@article{elucidating,
  title={Elucidating the design space of diffusion-based generative models},
  author={Karras, Tero and Aittala, Miika and Aila, Timo and Laine, Samuli},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={26565--26577},
  year={2022}
}

@inproceedings{alexnet,
author = {Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E.},
title = {ImageNet Classification with Deep Convolutional Neural Networks},
year = {2012},
publisher = {Curran Associates Inc.},
address = {Red Hook, NY, USA},
booktitle = {Proceedings of the 25th International Conference on Neural Information Processing Systems - Volume 1},
pages = {1097–1105},
numpages = {9},
location = {Lake Tahoe, Nevada},
series = {NIPS'12}
}

@InProceedings{adam,
  author    = {Kingma, Diederik and Ba, Jimmy},
  booktitle = {International Conference on Learning Representations (ICLR)},
  title     = {Adam: A Method for Stochastic Optimization},
  year      = {2015},
  address   = {San Diega, CA, USA},
  optmonth  = {12},
},





@string{cvgip  = {Computer Vision, Graphics and Image Processing}}
@string{spm    = {IEEE Signal Processing Magazine}}
@string{jmiv   = {Journal of Mathematical Imaging and Vision}}
@string{tpami  = {IEEE Transactions on Pattern Analysis and
                 Machine Intelligence}}
@string{lncs   = {Lecture Notes in Computer Science}}

@inproceedings{resnet,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}
,
@article{DiffBlockConn,
author = {Alt, Tobias and Schrader, Karl and Augustin, Matthias and Peter, Pascal and Weickert, Joachim},
title = {Connections Between Numerical Algorithms for PDEs and Neural Networks},
year = {2022},
issue_date = {Jan 2023},
publisher = {Kluwer Academic Publishers},
address = {USA},
volume = {65},
number = {1},
issn = {0924-9907},
journal = jmiv,
month = {jun},
pages = {185–208},
numpages = {24},
keywords = {Neural networks, Stability, Numerical algorithms, Partial differential equations, Nonlinear diffusion}
}
,
@inproceedings{DiffBlocktranslating,
author = {Alt, Tobias and Peter, Pascal and Weickert, Joachim and Schrader, Karl},
title = {Translating Numerical Concepts for PDEs into Neural Architectures},
year = {2021},
isbn = {978-3-030-75548-5},
publisher = {Springer-Verlag},
address = {Berlin, Heidelberg},
booktitle = {Scale Space and Variational Methods in Computer Vision: 8th International Conference, SSVM 2021, Virtual Event, May 16–20, 2021, Proceedings},
pages = {294–306},
numpages = {13},
keywords = {Convolutional neural networks, Nonlinear diffusion, Stability, Numerical algorithms, Partial differential equations}
},

@inproceedings{FSI,
  title={FSI schemes: Fast semi-iterative solvers for {PDE}s and optimisation methods},
  author={Hafner, David and Ochs, Peter and Weickert, Joachim and Rei{\ss}el, Martin and Grewenig, Sven},
  booktitle={Pattern Recognition: 38th German Conference, GCPR 2016, Hannover, Germany, September 12-15, 2016, Proceedings 38},
  pages={91--102},
  year={2016},
  organization={Springer}
},
@inproceedings{relu,
author = {Nair, Vinod and Hinton, Geoffrey E.},
title = {Rectified Linear Units Improve Restricted Boltzmann Machines},
year = {2010},
isbn = {9781605589077},
publisher = {Omnipress},
address = {Madison, WI, USA},
booktitle = {Proceedings of the 27th International Conference on Machine Learning},
pages = {807–814},
numpages = {8},
location = {Haifa, Israel},
series = {ICML'10}
},
@book{anisodiffweick,
  added-at = {2019-03-09T02:01:20.000+0100},
  author = {Weickert, Joachim},
  biburl = {https://www.bibsonomy.org/bibtex/2ecf195c5848a8339688f09c056092d48/kirk86},
  description = {book.pdf},
  interhash = {83398a0f353ad019469433981cf105a2},
  intrahash = {ecf195c5848a8339688f09c056092d48},
  keywords = {book diffusion image-processing physics stats},
  timestamp = {2020-01-29T21:38:53.000+0100},
  title = {Anisotropic Diffusion in Image Processing},
  url = {https://www.mia.uni-saarland.de/weickert/Papers/book.pdf},
  year = 1998,
  publisher	= {Teubner Stuttgart}
},
@inproceedings{eed,
author = {Weickert, Joachim},
title = {Theoretical Foundations of Anisotropic Diffusion in Image Processing},
year = {1994},
isbn = {3211827307},
publisher = {Springer-Verlag},
address = {Berlin, Heidelberg},
booktitle = {Proceedings of the 7th TFCV on Theoretical Foundations of Computer Vision},
pages = {221–236},
numpages = {16}
},
@inproceedings{eedcompr,
  title={Colour image compression with anisotropic diffusion},
  author={Peter, Pascal and Weickert, Joachim},
  booktitle={2014 IEEE International Conference on Image Processing (ICIP)},
  pages={4822--4826},
  year={2014},
  organization={IEEE}
}
,
@article{eedSuperior,
author = {Schmaltz, Christian and Peter, Pascal and Mainberger, Markus and Ebel, Franziska and Weickert, Joachim and Bruhn, Andr\'{e}s},
title = {Understanding, Optimising, and Extending Data Compression with Anisotropic Diffusion},
year = {2014},
issue_date = {July      2014},
publisher = {Kluwer Academic Publishers},
address = {USA},
volume = {108},
number = {3},
issn = {0920-5691},
journal = {International Journal of Computer Vision},
month = {jul},
pages = {222–240},
numpages = {19},
keywords = {Image compression, Subdivision, Kanizsa triangle, JPEG 2000, Partial differential equations (PDEs), Edge-enhancing anisotropic diffusion (EED)}
},
@inproceedings{Unet,
  title={U-net: Convolutional networks for biomedical image segmentation},
  author={Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas},
  booktitle={Medical Image Computing and Computer-Assisted Intervention--MICCAI 2015: 18th International Conference, Munich, Germany, October 5-9, 2015, Proceedings, Part III 18},
  pages={234--241},
  year={2015},
  organization={Springer}
},
@inproceedings{WWW,
  title={L2-stable nonstandard finite differences for anisotropic diffusion},
  author={Weickert, Joachim and Welk, Martin and Wickert, Marco},
  booktitle={Scale Space and Variational Methods in Computer Vision},
  volume={7893},
  pages={380--391},
  year={2013},
  organization={Springer}
}
,
@book{goodfellow,
  title={Deep learning},
  author={Goodfellow, Ian and Bengio, Yoshua and Courville, Aaron},
  year={2016},
  publisher={MIT press}
}
@inproceedings{wgain,
author = {Va\v{s}ata, Daniel and Halama, Tom\'{a}\v{s} and Friedjungov\'{a}, Magda},
title = {Image Inpainting Using Wasserstein Generative Adversarial Imputation Network},
year = {2021},
isbn = {978-3-030-86339-5},
publisher = {Springer-Verlag},
address = {Berlin, Heidelberg},
booktitle = {Artificial Neural Networks and Machine Learning – ICANN 2021: 30th International Conference on Artificial Neural Networks, Bratislava, Slovakia, September 14–17, 2021, Proceedings, Part II},
pages = {575–586},
numpages = {12},
keywords = {Image inpainting, Generative models, Wasserstein GAIN, Imputation methods, Missing data, Wasserstein GAN},
location = {Bratislava, Slovakia}
}
,
@inproceedings{flyingthings,
  title={A large dataset to train convolutional networks for disparity, optical flow, and scene flow estimation},
  author={Mayer, Nikolaus and Ilg, Eddy and Hausser, Philip and Fischer, Philipp and Cremers, Daniel and Dosovitskiy, Alexey and Brox, Thomas},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={4040--4048},
  year={2016}
},

@inproceedings{flownet,
author = {Dosovitskiy, Alexey and Fischery, Philipp and Ilg, Eddy and Hausser, Philip and Hazirbas, Caner and Golkov, Vladimir and Smagt, Patrick van der and Cremers, Daniel and Brox, Thomas},
title = {FlowNet: Learning Optical Flow with Convolutional Networks},
year = {2015},
isbn = {9781467383912},
publisher = {IEEE Computer Society},
address = {USA},
booktitle = {Proceedings of the 2015 IEEE International Conference on Computer Vision (ICCV)},
pages = {2758–2766},
numpages = {9},
series = {ICCV '15}
},
@inproceedings{Sintel,
author = {Butler, Daniel J. and Wulff, Jonas and Stanley, Garrett B. and Black, Michael J.},
title = {A Naturalistic Open Source Movie for Optical Flow Evaluation},
year = {2012},
isbn = {9783642337826},
publisher = {Springer-Verlag},
address = {Berlin, Heidelberg},
booktitle = {Proceedings of the 12th European Conference on Computer Vision - Volume Part VI},
pages = {611–625},
numpages = {15},
location = {Florence, Italy},
series = {ECCV'12}
}
@article{peronamalik,
author = {Perona, Pietro and Malik, Jitendra},
title = {Scale-Space and Edge Detection Using Anisotropic Diffusion},
year = {1990},
issue_date = {July 1990},
publisher = {IEEE Computer Society},
address = {USA},
volume = {12},
number = {7},
issn = {0162-8828},
journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
month = {jul},
pages = {629–639},
numpages = {11},
keywords = {anisotropic diffusion, intraregion smoothing, scale-space, edge detection, parallel processing, filtering and prediction theory, pattern recognition, picture processing}
},

@article{Di86,
  author =       {{Di Zenzo}, Silvano },
  title =        {A note on the gradient of a multi-image},
  journal =      cvgip,
  volume =       {33},
  number =       {},
  pages =        {116--125},
  month =        {},
  year =         {1986},
  note =         {}
}

@inproceedings{MM98a,
  author =       {Masnou, Simon and Morel, Jean-Michel},
  title =        {Level lines based disocclusion},
  editor =       {},
  booktitle =    {Proc.~1998 IEEE International Conference on Image
                 Processing},
  address =      {Chicago, IL},
  month =        oct,
  year =         {1998},
  pages =        {259--263},
  series =       {},
  volume =       {3},
  institution =  {},
  publisher =     {},
  note =         {}
}

@inproceedings{BSCB00,
  author =       {Bertalm\'io, Marcelo and Sapiro, Guillermo and Caselles, Vincent and
                 Ballester, Coloma},
  title =        {Image inpainting},
  editor =       {},
  booktitle =    {Proc. {SIGGRAPH} 2000},
  address =      {New Orleans, LI},
  month =        jul,
  year =         {2000},
  pages =        {417--424},
  series =       {},
  volume =       {},
  institution =  {},
  publisher =    {},
  note =         {}
}

@article{GL14,
  author =       {Guillemot, Christine and {Le Meur}, Olivier},
  title =        {Image inpainting: Overview and recent advances},
  journal =      spm,
  volume =       {31},
  number =       {1},
  pages =        {127--144},
  month =        {},
  year =         {2014},
  note =         {},
  annote =       {}
}

@inproceedings{AW21,
  author =       {Alt, Tobias and Weickert, Joachim},
  title  =       {Learning Integrodifferential Models for Denoising},
  editor =       {},
  booktitle =    {Proc.~2021 IEEE International Conference on Acoustics, Speech
                 and Signal Processing},
  address =      {Toronto, Canada},
  month =        jun, 
  year =         {2021},
  pages =        {2045--2049},
  series =       {},
  volume =       {},
  institution =  {},
  publisher =    {IEEE Computer Society Press},
  note =         {},
}

@article{CP16,
  author =       {Chen, Yunjin and Pock, Thomas},
  title =        {Trainable nonlinear reaction diffusion: A flexible 
                 framework for fast and effective image restoration},
  journal =      tpami,
  volume =       {39},
  number =       {6},
  pages =        {1256--1272},
  month =        aug,
  year =         {2016},
  note =         {}
}

@article{AH20,
  author =       {Arridge, Simon and Hauptmann, Andreas},
  title =        {Networks for Nonlinear Diffusion Problems in Imaging},
  journal =      jmiv,
  volume =       {62},
  number =       {},
  pages =        {471--487},
  month =        apr,
  year =         {2020},
  note =         {}
}


@inproceedings{JPW20,
  author =       {Jost, Ferdinand and Peter, Pascal and Weickert, Joachim},
  title =        {Compressing flow fields with edge-aware homogeneous diffusion 
                  inpainting},
  editor =       {},
  booktitle =    {Proc.~45th International Conference on Acoustics, Speech, and 
                  Signal Processing},
  address =      {Barcelona, Spain},
  month =        may,
  year =         {2020},
  pages =        {2198--2202},
  series =       {},
  volume =       {},
  institution =  {},
  publisher =    {IEEE Computer Society Press},
  note =         {}
}

@incollection{APMW21,
  author =       {Andris, Sarah and Peter, Pascal and Mohideen, Rahul and Weickert, Joachim 
                  and Hoffmann, Sebastian},
  title =        {Inpainting-based video compression in {FullHD}},
  editor =       {A. Elmoataz and J. Fadili and Y. Qu\'eau and J. Rabin and L. 
                  Simon},
  booktitle =    {Scale Space and Variational Methods in Computer Vision},
  chapter =      {},
  pages =        {425--436},
  series =       lncs,
  volume =       {12679},
  number =       {},
  institution =  {},
  publisher =    {Springer},
  address =      {Cham},
  month =        {},
  year =         {2021},
  note =         {},
  annote =       {}
},
@article{imagen,
  title={Photorealistic Text-to-Image Diffusion Models with Deep Language Understanding},
  author={Saharia, Chitwan and Chan, William and Saxena, Saurabh and Li, Lala and Whang, Jay and Denton, Emily L and Ghasemipour, Kamyar and Gontijo Lopes, Raphael and Karagol Ayan, Burcu and Salimans, Tim and others},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={36479--36494},
  year={2022}
},

@inproceedings{repaint,
  title={Repaint: Inpainting using denoising diffusion probabilistic models},
  author={Lugmayr, Andreas and Danelljan, Martin and Romero, Andres and Yu, Fisher and Timofte, Radu and Van Gool, Luc},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={11461--11471},
  year={2022}
},

@inproceedings{flownet2,
  title={Flownet 2.0: Evolution of optical flow estimation with deep networks},
  author={Ilg, Eddy and Mayer, Nikolaus and Saikia, Tonmoy and Keuper, Margret and Dosovitskiy, Alexey and Brox, Thomas},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2462--2470},
  year={2017}
},

@article{stabilityy,
  title={Properties of higher order nonlinear diffusion filtering},
  author={Didas, Stephan and Weickert, Joachim and Burgeth, Bernhard},
  journal=jmiv,
  volume={35},
  pages={208--226},
  year={2009},
  publisher={Springer}
},
@inproceedings{realTimeHom,
  title={Domain Decomposition Algorithms for Real-Time Homogeneous Diffusion Inpainting in 4K},
  author={K{\"a}mper, Niklas and Weickert, Joachim},
  booktitle={Proceedings of the IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={1680--1684},
  year={2022},
  organization={IEEE}
},
@book{differences,
  title={Numerical Solution of Partial Differential Equations: An Introduction},
  author={Morton, Keith W and Mayers, David Francis},
  year={2005},
  publisher={Cambridge university press}
},
@inproceedings{neuralode,
author = {Chen, Ricky T. Q. and Rubanova, Yulia and Bettencourt, Jesse and Duvenaud, David},
title = {Neural Ordinary Differential Equations},
year = {2018},
publisher = {Curran Associates Inc.},
address = {Red Hook, NY, USA},
booktitle = {Proceedings of the 32nd International Conference on Neural Information Processing Systems},
pages = {6572–6583},
numpages = {12},
location = {Montr\'{e}al, Canada},
series = {NIPS'18}
}
,
@article{chenpock,
author = {Chen, Yunjin and Pock, Thomas},
title = {Trainable Nonlinear Reaction Diffusion: A Flexible Framework for Fast and Effective Image Restoration},
year = {2017},
issue_date = {June 2017},
publisher = {IEEE Computer Society},
address = {USA},
volume = {39},
number = {6},
issn = {0162-8828},
journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
month = {jun},
pages = {1256–1272},
numpages = {17}
}
,
@article{ruthotto1,
  title={Stable Architectures for Deep Neural Networks},
  author={Haber, Eldad and Ruthotto, Lars},
  journal={Inverse Problems},
  volume={34},
  number={1},
  article={014004},
  year={2017},
  publisher={IOP Publishing}
},
@article{ruthotto2,
  title={Deep neural networks motivated by partial differential equations},
  author={Ruthotto, Lars and Haber, Eldad},
  journal={Journal of Mathematical Imaging and Vision},
  volume={62},
  pages={352--364},
  year={2020},
  publisher={Springer}
},

@article{multigrid,
  title={Multi-level adaptive solutions to boundary-value problems},
  author={Brandt, Achi},
  journal={Mathematics of Computation},
  volume={31},
  number={138},
  pages={333--390},
  year={1977}
},
@inproceedings{raft,
author = {Teed, Zachary and Deng, Jia},
title = {RAFT: Recurrent All-Pairs Field Transforms for Optical Flow},
year = {2020},
month= {August},
isbn = {978-3-030-58535-8},
publisher = {Springer-Verlag},
address = {Berlin, Heidelberg},
booktitle = {Proceedings of the 12th European Conference on Computer Vision -- Volume Part II},
pages = {402–419},
numpages = {18},
location = {Glasgow, United Kingdom}
}
@inproceedings{gmflow,
  title={Gmflow: Learning Optical Flow via Global Matching},
  author={Xu, Haofei and Zhang, Jing and Cai, Jianfei and Rezatofighi, Hamid and Tao, Dacheng},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={8121--8130},
  year={2022}
},
@inproceedings{flowformer,
author = {Huang, Zhaoyang and Shi, Xiaoyu and Zhang, Chao and Wang, Qiang and Cheung, Ka Chun and Qin, Hongwei and Dai, Jifeng and Li, Hongsheng},
title = {FlowFormer: A Transformer Architecture For Optical Flow},
year = {2022},
month = {October},
isbn = {978-3-031-19789-5},
publisher = {Springer-Verlag},
address = {Berlin, Heidelberg},
booktitle = {Proceedings of the 17th European Conference on Computer Vision -- Volume Part XVII},
pages = {668–685},
numpages = {18},
keywords = {Optical flow, Transformer, Cost volume, RAFT},
location = {Tel Aviv, Israel}
},
@article{weickertschnoerr,
author = {Weickert, Joachim and Schn\"{o}rr, Christoph},
title = {A Theoretical Framework for Convex Regularizers in PDE-Based Computation of Image Motion},
year = {2001},
issue_date = {December 2001},
publisher = {Kluwer Academic Publishers},
address = {USA},
volume = {45},
number = {3},
issn = {0920-5691},
journal = {International Journal of Computer Vision},
month = {December},
pages = {245–264},
numpages = {20},
keywords = {optic flow, regularization, well-posedness, diffusion filtering, differential methods}
},

@misc{vkitti2,
  title={Virtual KITTI 2},
  author={Cabon, Yohann and Murray, Naila and Humenberger, Martin},
  year={2020},
  eprint={2001.10773},
  archivePrefix={arXiv},
  primaryClass={cs.CV}
},
@inproceedings{vkitti,
  title={Virtual worlds as proxy for multi-object tracking analysis},
  author={Gaidon, Adrien and Wang, Qiao and Cabon, Yohann and Vig, Eleonora},
  booktitle={Proceedings of the IEEE conference on Computer Vision and Pattern Recognition},
  pages={4340--4349},
  year={2016}
}





























































